Universal nature of the nonlinear stage of modulational instability

We characterize the nonlinear stage of modulational instability (MI) by studying the long-time asymptotics of focusing nonlinear Schrodinger (NLS) equation on the infinite line with initial conditions that tend to constant values at infinity. Asymptotically in time, the spatial domain divides into three regions: a far left field and a far right field, in which the solution is approximately equal to its initial value, and a central region in which the solution has oscillatory behavior and is described by slow modulations of the periodic traveling wave solutions of the focusing NLS equation. These results demonstrate that the asymptotic stage of MI is universal, since the long-time behavior of a large class of perturbations is described by the same asymptotic state.

==> references.tex <==
\catcode`\@ 11
\def\journal#1&#2,#3 (#4){\begingroup \let\journal=\d@mmyjournal {\frenchspacing\sl #1\/\unskip\,} {\bf\ignorespaces #2}\rm,\ #3 (#4)\endgroup}
\def\d@mmyjournal{\errmessage{Reference foul up: nested \journal macros}}
\def\@biblabel#1{#1.}
\begin{thebibliography}O
\def\booktitle#1{\textsl{#1}}
\def\journal#1&#2,{\textrm{#1}\textbf{#2},}
\itemsep 0pt


\kern-\medskipamount

\item[*] Electronic address: biondini@buffalo.edu.~\ 

\bibitem{zakharovostrovsky}
V.E. Zakharov and L.A. Ostrovsky, 
\reftitle{Modulational instability: the beginning}, Phys. D \textbf{238} 540 (2009)

\bibitem{benjaminfeir}
T.B. Benjamin and J.E. Feir, 
\reftitle{The disintegration of wave trains on deep water}, 
J. Fluid Mech. \textbf{27}, 417  (1967)

\bibitem{naturephys}
B. Kibler \etalii{J. Fatome, C. Finot, G. Millot, F. Dias, G. Genty, N. Akhmediev and J.M. Dudley}, 
\reftitle{The Peregrine soliton in nonlinear fibre optics}, 
Nat. Phys. \textbf6, 790 (2010)

\bibitem{solli}
D.R. Solli \etalii{C. Ropers, P. Koonath and B. Jalali},
\reftitle{Optical rogue waves},
Nature \textbf{450}, 1054 (2007)

\bibitem{onoratoosborne}
M. Onorato, A.R. Osborne and M. Serio,
\reftitle{Modulational instability in crossing sea states: A possible mechanism for the formation of freak waves},
Phys. Rev. Lett. \textbf{96}, 014503 (2006)

\bibitem{zakharovshabat1972}
V.E. Zakharov and A.B. Shabat,
\reftitle{Exact theory of two-dimensional self-focusing and one-dimensional self-modulation of waves in nonlinear media},
\journal Sov. Phys. JETP &34, 62 (1972)

\bibitem{zakharovgelash}
V.E. Zakharov and A.A. Gelash,
\reftitle{Nonlinear stage of modulation instability},
Phys. Rev. Lett. \textbf{111}, 054101 (2013)

\bibitem{gelash}
A.A. Gelash and V.E. Zakharov, 
\reftitle{Superregular solitonic solutions: a novel scenario for the nonlinear stage of modulation instability},
Nonlinearity \textbf{27}, 1 (2014)

\bibitem{zakharovshabat1973}
V.E. Zakharov and A.B. Shabat,
\reftitle{Interaction between solitons in a stable medium},
\journal Sov. Phys. JETP &37, 823 (1973)

\bibitem{kuznetsov}
E.A. Kuznetsov, 
\reftitle{Solitons in a parametrically unstable plasma}, 
Sov. Phys. Dokl. \textbf{22}, 507  (1977)

\bibitem{ma}
Y.-C. Ma, 
\reftitle{The perturbed plane-wave solutions of the cubic Schr\"odinger equation},
Stud. Appl. Math. \textbf{60}, 43-- 58 (1979)

\bibitem{garnier}
J. Garnier and K. Kalimeris,
\reftitle{Inverse scattering perturbation theory for the nonlinear Schr\"odinger equation with non-vanishing background},
J. Phys. A \textbf{45}, 035202 (2012)

\bibitem{biondinikovacic}
G. Biondini and G. Kova\v{c}i\v{c},
\reftitle{Inverse scattering transform for the focusing nonlinear Schr\"odinger equation with nonzero boundary conditions},
\journal J. Math. Phys. &55, 031506 (2014)

\bibitem{prinari}
B. Prinari, M.J. Ablowitz and G. Biondini,
\reftitle{Inverse scattering transform for the vector nonlinear Schr\"odinger equation with non-vanishing boundary conditions},
\journal J. Math. Phys. &47, 063508 (2006)

\bibitem{kbk2015}
D.K. Kraus, G. Biondini and G. Kova\v{c}i\v{c},
\reftitle{The focusing Manakov system with nonzero boundary conditions},
\journal Nonlinearity &28, 3101 (2015)

\bibitem{biondinifagerstrom}
G. Biondini and E.R. Fagerstrom, 
\reftitle{Integrable nature of modulational instability},
SIAM J. Appl. Math. \textbf{75}, 136 (2015)

\bibitem{peregrine}
D.H. Peregrine, 
\reftitle{Water waves, nonlinear Schr\"odinger equations and their solutions}, 
Austral. Math. Soc. Ser. B \textbf{25}, 16 (1983)

\bibitem{akhmediev}
N.N. Akhmediev and V.I. Korneev,
\reftitle{Modulational instability and periodic solutions of the nonlinear Schr\"odinger equation},
Theor. Math. Phys. \textbf{69}, 1089 (1987)

\bibitem{tajiriwatanabe}
M. Tajiri and Y. Watanabe, 
\reftitle{Breather solutions to the focusing nonlinear Schr\"odinger equation}, 
Phys. Rev. E \textbf{57}, 3510 (1998)

\bibitem{ablowitzherbst1990}
M.J. Ablowitz and B.M. Herbst,
\reftitle{On homoclinic structure and numerically induced chaos for the nonlinear Schr\"odinger equation},
SIAM J. Appl. Math. \textbf{50}, 339 (1990)

\bibitem{henderson1999}
K.L. Henderson, D.H. Peregrine and J.W. Dold,
\reftitle{Unsteady water wave modulations: Fully nonlinear solutions and comparison with the nonlinear Schr\"odinger equation},
Wave Motion \textbf{29}, 341 (1999)

\bibitem{whitham}
G.B. Whitham,
\textsl{Linear and nonlinear waves}
(Wiley, 1974)

\bibitem{ablowitzsegur1976}
H. Segur and M.J. Ablowitz,
\reftitle{Asymptotic solutions and conservation laws for the nonlinear Schr\"odinger equation},
J. Math. Phys. \textbf{17}, 710 (1976) 

\bibitem{zakharovmanakov}
V.E. Zakharov and S.V. Manakov,
\reftitle{Asymptotic behavior of nonlinear waves systems integrated by the inverse scattering method},
Sov. Phys. JETP \textbf{44} 106 (1976)

\bibitem{deiftzhou}
P. Deift and X. Zhou,
\reftitle{A steepest descent method for oscillatory Riemann-Hilbert problems. Asymptotics for the mKdV equation}, 
Ann. Math. \textbf{137}, 295 (1993)

\bibitem{buckingham}
R. Buckingham and S. Venakides,
\reftitle{Long-time asymptotics of the nonlinear Schr\"odinger equation shock problem}, 
Commun. Pure Appl. Math. \textbf{40}, 1349 (2007)

\bibitem{boutet}
A. Boutet de Monvel, V.P. Kotlyarov and D. Shepelsky,
\reftitle{Focusing NLS equation: Long-time dynamics of step-like initial data}, 
Int. Math. Res. Not. \textbf{2011} 1613 (2011)

%\bibitem{whittakerwatson}
%E.T. Whittaker and G.N. Watson,
%\textit{A course of modern analysis} 
%(Cambridge University Press, 1950)

\bibitem{el}
G.A. El \etalii{A.V. Gurevich, V.V. Khodorovskii and A.L. Krylov},
\reftitle{Modulation instability and formation of a nonlinear oscillatory structure in a focusing medium},
Phys. Lett. A \textbf{177}, 357 (1993)

\bibitem{kamchatnov}
A.M. Kamchatnov,
\textit{Nonlinear periodic waves and their modulations}
(World Scientific, 2000)

\bibitem{prl71p2683}
M.J. Ablowitz, C.M. Schober and B.M. Herbst,
\reftitle{Numerical chaos, roundoff errors and homoclinic manifolds},
Phys. Rev. Lett. \textbf{71}, 2683 (1993)

\bibitem{Trillo1}
S. Trillo and S. Wabnitz,
\reftitle{Dynamics of the nonlinear modulational instability in optical fibers},
Opt. Lett. \textbf{16}, 986 (1991)

\bibitem{itskotlyarov}
A.R. Its and V.P. Kotlyarov,
\title{Explicit formulas for solutions of the NLS equation},
Dokl. Akad. Nauk Ukr. SSR A \textbf{11}, 965 (1965)

\bibitem{maablowitz}
Y.-C. Ma and M.J. Ablowitz, 
\reftitle{The periodic cubic NLS equation},
Stud. Appl. Math. \textbf{63}, 113 (1981)

\bibitem{KMM}
S. Kamvissis, K.D. McLaughlin and P.D. Miller,
\textit{Semiclassical soliton ensembles for the focusing nonlinear Schrödinger equation}
(Princeton University Press, 2003)

\bibitem{zakharov2009}
V.E. Zakharov, 
\reftitle{Turbulence in integrable systems}, 
Stud. Appl. Math. \textbf{122}, 219 (2009)

%\bibitem{AS1981}
%M.~J. Ablowitz and H. Segur, 
%{\em Solitons and the inverse scattering transform}
%(SIAM, Philadelphia, 1981)

%\bibitem{ggkm1967}
%* C.S. Gardner, C.S. Greene, M.D. Kruskal and R.M. Miura, 
%\reftitle{Method for Solving the Korteweg-de Vries Equation}, 
%\journal Phys. Rev. Lett. &19, 1095 (1967)

%\bibitem{Trillo2}
%S. Trillo, S. Wabnitz and T.A.B. Kennedy,
%\reftitle{Nonlinear dynamics of dual-frequency-pumped multiwave mixing in optical fibers},
%Phys. Rev. A \textbf{50}, 1732 (1994)

%\bibitem{sapm2011}
%* B. Prinari, G. Biondini and A.D. Trubatch,
%\reftitle{Inverse scattering transform for the multi-component nonlinear Schr\"odinger equation with nonzero boundary conditions},
%\journal Stud. Appl. Math. &126, 245 (2011)
% ist for multicomponent VNLS w/ NZBC


\end{thebibliography}

